TTPXHunter: Actionable Threat Intelligence Extraction as TTPs from Finished Cyber Threat Reports

Understanding the modus operandi of adversaries aids organizations in employing efficient defensive strategies and sharing intelligence in the community. This knowledge is often present in unstructured natural language text within threat analysis reports. A translation tool is needed to interpret the modus operandi explained in the sentences of the threat report and translate it into a structured format. This research introduces a methodology named TTPXHunter for the automated extraction of threat intelligence in terms of Tactics, Techniques, and Procedures (TTPs) from finished cyber threat reports. It leverages cyber domain-specific state-of-the-art natural language processing (NLP) to augment sentences for minority class TTPs and refine pinpointing the TTPs in threat analysis reports significantly. The knowledge of threat intelligence in terms of TTPs is essential for comprehensively understanding cyber threats and enhancing detection and mitigation strategies. We create two datasets: an augmented sentence-TTP dataset of 39,296 samples and a 149 real-world cyber threat intelligence report-to-TTP dataset. Further, we evaluate TTPXHunter on the augmented sentence dataset and the cyber threat reports. The TTPXHunter achieves the highest performance of 92.42% f1-score on the augmented dataset, and it also outperforms existing state-of-the-art solutions in TTP extraction by achieving an f1-score of 97.09% when evaluated over the report dataset. TTPXHunter significantly improves cybersecurity threat intelligence by offering quick, actionable insights into attacker behaviors. This advancement automates threat intelligence analysis, providing a crucial tool for cybersecurity professionals fighting cyber threats.

==> Reference.tex <==
\bibitem{Rani2023TTPHunter}
Nanda Rani, Bikash Saha, Vikas Maurya, and Sandeep Kumar Shukla. "TTPHunter: Automated Extraction of Actionable Intelligence as TTPs from Narrative Threat Reports." In \textit{Proceedings of the 2023 Australasian Computer Science Week}, pp. 126--134, 2023.

\bibitem{Aghaei2023SecureBERT}
Ehsan Aghaei, Xi Niu, Waseem Shadid, and Ehab Al-Shaer. "SecureBERT: A Domain-Specific Language Model for Cybersecurity." In \textit{International Conference on Security and Privacy in Communication Systems}, pp. 39--56. Springer, 2022.

\bibitem{alam2023looking}
Md Tanvirul Alam, Dipkamal Bhusal, Youngja Park, and Nidhi Rastogi. "Looking beyond IoCs: Automatically extracting attack patterns from external CTI." In \textit{Proceedings of the 26th International Symposium on Research in Attacks, Intrusions and Defenses}, pp. 92--108, 2023.

\bibitem{Husari2017Ttpdrill}
Ghaith Husari, Ehab Al-Shaer, Mohiuddin Ahmed, Bill Chu, and Xi Niu. "Ttpdrill: Automatic and accurate extraction of threat actions from unstructured text of cti sources." In \textit{Proceedings of the 33rd annual computer security applications conference}, pp. 103--115, 2017.

\bibitem{Li2022AttacKG}
Zhenyuan Li, Jun Zeng, Yan Chen, and Zhenkai Liang. "AttacKG: Constructing technique knowledge graph from cyber threat intelligence reports." In \textit{European Symposium on Research in Computer Security}, pp. 589--609. Springer, 2022.

\bibitem{MITREATTACK}
MITRE. "ATT\&CK Framework." 2023. Available online: \url{https://attack.mitre.org}. [Accessed July 22, 2023].

\bibitem{HuggTrans}
Hugging Face. Transformers, 2024.  Available online: \url{https://huggingface.co/docs/transformers/en/index}

\bibitem{Tram}
MITRE. "Threat Report ATT\&CK Mapper (TRAM)." 2023. Available online: \url{https://github.com/center-for-threat-informed-defense/tram/}. [Accessed Feb 22, 2024].

\bibitem{legoy2020automated}
Valentine Legoy, Marco Caselli, Christin Seifert, and Andreas Peter. "Automated retrieval of att\&ck tactics and techniques for cyber threat reports." \textit{arXiv preprint arXiv:2004.14322}, 2020.

\bibitem{scikit-learn}
F. Pedregosa, G. Varoquaux, A. Gramfort, V. Michel, B. Thirion, O. Grisel, M. Blondel, P. Prettenhofer, R. Weiss, V. Dubourg, J. Vanderplas, A. Passos, D. Cournapeau, M. Brucher, M. Perrot, and E. Duchesnay,
"Scikit-learn: Machine Learning in \{P\}ython," \textit{Journal of Machine Learning Research}, vol. 12, pp. 2825--2830, 2011.

\bibitem{Reimers2019Sentence}
Nils Reimers and Iryna Gurevych.
\newblock Sentence-bert: Sentence embeddings using siamese bert-networks.
\newblock \emph{arXiv preprint arXiv:1908.10084}, 2019.

\bibitem{Vaswani2017Attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan N. Gomez, {\L}ukasz Kaiser, and Illia Polosukhin.
\newblock Attention is all you need.
\newblock \emph{Advances in neural information processing systems}, 30, 2017.

\bibitem{Rifat2022BERT}
Nafiz Rifat, Mostofa Ahsan, Md Chowdhury, and Rahul Gomes,
``BERT against social engineering attack: Phishing text detection,''
in \textit{2022 IEEE International Conference on Electro Information Technology (eIT)},
IEEE, 2022, pp. 1--6.

\bibitem{Tikhomirov2020Using}
M. Tikhomirov, N. Loukachevitch, A. Sirotina, and B. Dobrov,
``Using BERT and augmentation in named entity recognition for cybersecurity domain,''
in \textit{Natural Language Processing and Information Systems: 25th International Conference on Applications of Natural Language to Information Systems, NLDB 2020, Saarbr{\"u}cken, Germany, June 24--26, 2020, Proceedings 25},
Springer, 2020, pp. 16--24.

\bibitem{barnum2012standardizing}
S. Barnum, ``Standardizing cyber threat intelligence information with the structured threat information expression (STIX),'' \textit{Mitre Corporation}, vol. 11, pp. 1--22, 2012.

\bibitem{de2009tutorial}
A. C. P. L. F. de Carvalho and A. A. Freitas, ``A tutorial on multi-label classification techniques,'' in \textit{Foundations of Computational Intelligence Volume 5: Function Approximation and Classification}, Springer, 2009, pp. 177--195.

\bibitem{zhang2013review}
M.-L. Zhang and Z.-H. Zhou, ``A review on multi-label learning algorithms,'' \textit{IEEE Transactions on Knowledge and Data Engineering}, vol. 26, no. 8, pp. 1819--1837, 2013, IEEE.

\bibitem{beltagy2019scibert}
Beltagy, Iz and Lo, Kyle and Cohan, Arman. 
``SciBERT: A pretrained language model for scientific text.'' 
\textit{arXiv preprint arXiv:1903.10676}, 2019.

\bibitem{daszczyszak2019ttp}
Daszczyszak, Roman and Ellis, Dan and Luke, Steve and Whitley, Sean.
\newblock TTP-Based Hunting.
\newblock {\em MITRE CORP MCLEAN VA, Tech. Rep}, 2019.

\bibitem{Tang2022}
B. Tang, J. Wang, Z. Yu, B. Chen, W. Ge, J. Yu, and T. Lu,
"Advanced Persistent Threat intelligent profiling technique: A survey,"
\textit{Computers and Electrical Engineering}, vol. 103, pp. 108261, 2022, Elsevier.

\bibitem{rahman2022threat}
Rahman, Md Rayhanur and Williams, Laurie. "From Threat Reports to Continuous Threat Intelligence: A Comparison of Attack Technique Extraction Methods from Textual Artifacts." \textit{arXiv preprint arXiv:2210.02601} (2022).

\bibitem{saha2023malxcap}
Bikash Saha, Nanda Rani, and Sandeep Kumar Shukla.
\newblock MalXCap: A Method for Malware Capability Extraction.
\newblock In \textit{International Conference on Information Security Practice and Experience}, pages 230--249. Springer, 2023.



==> tables/ClasswiseMetrics.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{Precision Range} & \textbf{TTPXHunter} & \textbf{LADDER} & \textbf{ATTACKG} & \textbf{TRAM} & \textbf{RCATT} \\
    \hline
    \hline
    0-0.1 &	0 &	0 &	11 &	0 &	134\\
    \hline
    0.1-0.2 &	0 &	0 &	2 &	0 &	1 \\
    \hline
    0.2-0.3 &	0 &	0 &	4 &	1 &	0 \\
    \hline
    0.3-0.4 &	0 &	0 &	2 &	1 &	0 \\
    \hline
    0.4-0.5 &	0 &	1 &	2 &	2 &	0 \\
    \hline
    0.5-0.6 &	0 &	2 &	3 &	0 &	0 \\
    \hline
    0.6-0.7 &	0 &	4 &	4 &	6 &	0 \\
    \hline
    0.7-0.8 &	2 &	19 &	4 &	9 &	0 \\
    \hline
    0.8-0.9 &	8 &	36 &	0 &	17 &	0 \\
    \hline
    0.9-1.0 &	183 &	131 &	161 &	157 & 58 \\
    \hline
\end{tabular}

==> tables/ReportResultComparisonMicro.tex <==
\begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Model} & \textbf{Precision (\%)} & \textbf{Recall (\%)} & \textbf{F1-score (\%)} & \textbf{Hamming Loss} \\
    \hline
    \hline
     ATTACKG~\cite{Li2022AttacKG} & $89.18$ & $96.31$ & $92.61$ & $0.14$ \\
     \hline
     rcATT~\cite{legoy2020automated} & $31.93$ & $98.50$ & $48.22$ & $0.64$ \\
     \hline
     Ladder~\cite{alam2023looking} & $93.18$ & $96.06$ & $94.60$ & $0.10$ \\
     \hline
     TRAM~\cite{Tram}& $94.68$ & $94.45$ & $94.57$ & $0.10$  \\
     \hline
     % & & & & \\
     % \hline
     % & & & & \\
     % \hline
     \textbf{TTPXHunter (Proposed)} & $\textbf{97.48}$ & $\textbf{97.61}$ & $\textbf{97.55}$ & $\textbf{0.05}$\\
     \hline
\end{tabular}

==> tables/SentenceResultComparison.tex <==
\begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Model} & \textbf{Accuracy (\%)} & \textbf{Precision (\%)} & \textbf{Recall (\%)} & \textbf{F1-score (\%)} \\
    \hline
    \hline
     ATTACKG~\cite{Li2022AttacKG} & & & & \\
     \hline
     rcATT~\cite{legoy2020automated} & 19.38 & 20.89 & 16.22 & 14.13 \\
     \hline
     Ladder~\cite{alam2023looking} & & & & \\
     \hline
     TRAM~\cite{Tram}& 86.62 & 68.67 & 70.00 & 68.53 \\
     \hline
     % & & & & \\
     % \hline
     % & & & & \\
     % \hline
     \textbf{TTPXHunter (Proposed)} & $93.82$ & $94.01$ & $92.69$ & $92.42$ \\
     \hline
\end{tabular}
